Globally Interpretable Graph Learning via Distribution Matching

Graph neural networks (GNNs) have emerged as a powerful model to capture critical graph patterns. Instead of treating them as black boxes in an end-to-end fashion, attempts are arising to explain the model behavior. Existing works mainly focus on local interpretation to reveal the discriminative pattern for each individual instance, which however cannot directly reflect the high-level model behavior across instances. To gain global insights, we aim to answer an important question that is not yet well studied: how to provide a global interpretation for the graph learning procedure? We formulate this problem as globally interpretable graph learning, which targets on distilling high-level and human-intelligible patterns that dominate the learning procedure, such that training on this pattern can recover a similar model. As a start, we propose a novel model fidelity metric, tailored for evaluating the fidelity of the resulting model trained on interpretations. Our preliminary analysis shows that interpretative patterns generated by existing global methods fail to recover the model training procedure. Thus, we further propose our solution, Graph Distribution Matching (GDM), which synthesizes interpretive graphs by matching the distribution of the original and interpretive graphs in the GNN's feature space as its training proceeds, thus capturing the most informative patterns the model learns during training. Extensive experiments on graph classification datasets demonstrate multiple advantages of the proposed method, including high model fidelity, predictive accuracy and time efficiency, as well as the ability to reveal class-relevant structure.

==> table.tex <==
\begin{table*}[t]
\centering
% \footnotesize
\caption{\textbf{Model Fidelity} with a varying number of interpretive graphs generated per class. \lu{combine model fidelity and utility in the same table}}
% \resizebox{\columnwidth}{!}
{%
\renewcommand{\arraystretch}{.75}
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{Graphs/Cls} & \multicolumn{3}{c}{\textbf{Graph-Twitter}} & \multicolumn{3}{c}{\textbf{Graph-SST5}}  \\
\cmidrule(rl){2-4}\cmidrule(rl){5-7}
 & \ourmodel{} & GNNInterpreter & Random & \ourmodel{} & GNNInterpreter & Random & \\
\midrule
10 & \textbf{58.13 $\pm$ 2.74}  & 49.47 $\pm$ 0.96 & 46.59 $\pm$ 5.85 &  \textbf{36.62 $\pm$ 0.76} & 28.06 $\pm$ 0.33 & 29.33 $\pm$ 3.25 \\
50 & \textbf{59.73 $\pm$ 1.11} & 55.67 $\pm$ 1.04 & 50.20 $\pm$ 5.71 &   37.64 $\pm$ 0.83 & 35.96 $\pm$ 1.04  & \textbf{37.83 $\pm$ 3.62}\\
100 &  53.25 $\pm$1.30 & \textbf{59.76 $\pm$ 1.00} &  56.65 $\pm$ 2.78 &  \textbf{42.05 $\pm$ 1.35} & 41.04 $\pm$ 0.79  & 41.87 $\pm$ 1.80 \\
 & \multicolumn{3}{c}{{GCN Accuracy:61.40}} & \multicolumn{3}{c}{{GCN Accuracy:44.39}}  \\
\midrule

 & \multicolumn{3}{c}{\textbf{BA-Motif}} & \multicolumn{3}{c}{\textbf{BA-LRP}}  \\
\cmidrule(rl){2-4}\cmidrule(rl){5-7}
 & \ourmodel{} & GNNInterpreter & Random & \ourmodel{} & GNNInterpreter & Random & \\
\midrule
1 &  \textbf{73.00 $\pm$ 7.38}  & 61.2 $\pm$ 8.08 & 67.60 $\pm$ 4.52 & 
\textbf{64.72 $\pm$ 4.44} & 49.52 $\pm$ 0.43 &  51.12 $\pm$ 2.50 \\
5 & \textbf{89.00 $\pm$ 1.67}& 83.4 $\pm $10.67 & 49.60$\pm$1.96 &  \textbf{85.50 $\pm$ 2.05} & 79.01 $\pm$ 1.35  & 49.87 $\pm$ 1.28\\
10 &  \textbf{91.60 $\pm$ 3.72} & 79.01 $\pm$ 1.34 &  50.60 $\pm$ 1.56 & \textbf{95.50 $\pm$ 0.50} & 56.97 $\pm$ 1.10  & 52.38 $\pm$ 1.79  \\
 & \multicolumn{3}{c}{{GCN Accuracy: 100.00}} & \multicolumn{3}{c}{{GCN Accuracy: 97.95}}  \\
  \midrule
  
 & \multicolumn{3}{c}{\textbf{MUTAG}} & \multicolumn{3}{c}{\textbf{Shape}}  \\
\cmidrule(rl){2-4}\cmidrule(rl){5-7}
 & \ourmodel{} & GNNInterpreter & Random & \ourmodel{} & GNNInterpreter & Random & \\
\cmidrule(rl){2-4}\cmidrule(rl){5-7}
1 & \textbf{81.05 $\pm$ 9.76} & 79.53 $\pm$ 2.58 & 49.47 $\pm$ 10.84 &   \textbf{32.00 $\pm$ 4.00} & 20.00 $\pm$ 0.00 & 26.00 $\pm$ 12.00\\
5 & \textbf{92.63 $\pm$ 2.58} & 84.21 $\pm$ 0.00 & 65.26 $\pm$ 6.31 &    \textbf{88.00 $\pm$ 9.80} & 60.00 $\pm$ 0.00  & 48.00 $\pm$ 7.50\\
10 &  \textbf{94.73 $\pm$ 0.00} & 85.26 $\pm$ 6.14 &  66.31$\pm$5.37 &   \textbf{84.00 $\pm$ 8.00} & 62.00 $\pm$ 7.48  & 48.00 $\pm$ 4.00  \\
& \multicolumn{3}{c}{{GCN Accuracy:88.63}} & \multicolumn{3}{c}{{GCN Accuracy:100.00}}  \\
\bottomrule
\end{tabular}
}
\label{tab:train-time}
\end{table*}





\begin{table*}
% \footnotesize
\caption{\textbf{Model Fidelity} with a varying number of interpretive graphs generated per class.}
% \resizebox{\columnwidth}{!}
{%
% \renewcommand{\arraystretch}{.75}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Graphs/Cls} & \multicolumn{3}{c}{\textbf{Model Fidelity}} & \multicolumn{3}{c}{\textbf{Model Utility}} & \multirow{2}{*}{GCN Accuracy} \\
\cmidrule(rl){3-5}\cmidrule(rl){6-8}
&  & GDM & GNNInterpreter & Random & GDM & GNNInterpreter & Random & \\
\midrule

\multirow{3}{*}{MUTAG} 
& 1 & \textbf{81.05 $\pm$ 9.76} & 79.53 $\pm$ 2.58 & 49.47 $\pm$ 10.84 &  
\textbf{71.92 $\pm$ 2.48} & 70.17 $\pm$ 2.48 & 50.87$\pm$ 15.0 & \multirow{3}{*}{88.63} \\
& 5 & \textbf{92.63 $\pm$ 2.58} & 84.21 $\pm$ 0.00 & 65.26 $\pm$ 6.31 &
77.19 $\pm$ 4.96 & 57.89 $\pm$ 4.29 & \textbf{80.70 $\pm$  2.40} \\
& 10 &  \textbf{94.73 $\pm$ 0.00} & 85.26 $\pm$ 6.14 &  66.31$\pm$5.37  &
\textbf{82.45 $\pm$ 2.48} & 59.65 $\pm$ 8.94  &  75.43 $\pm$ 6.56 \\
\midrule
\multirow{3}{*}{Shape} 
& 1 & \textbf{32.00 $\pm$ 4.00} & 20.00 $\pm$ 0.00 & 26.00 $\pm$ 12.00 &  
\textbf{93.33 $\pm$ 4.71} & 60.00  $\pm$ 7.49 & 33.20 $\pm$ 4.71 & \multirow{3}{*}{100.00} \\
& 5 & \textbf{88.00 $\pm$ 9.80} & 60.00 $\pm$ 0.00  & 48.00 $\pm$ 7.50 &
\textbf{96.66 $\pm$ 4.71} & 85.67 $\pm$ 2.45  & 85.39  $\pm$  12.47 \\
& 10 &  \textbf{84.00 $\pm$ 8.00} & 62.00 $\pm$ 7.48  & 48.00 $\pm$ 4.00  &
\textbf{100.00  $\pm$ 0.00} & 88.67 $\pm$ 4.61  & 87.36  $\pm$  4.71 \\
\midrule
\multirow{3}{*}{\textbf{BA_Motif}}
& 1 & \textbf{73.00 $\pm$ 7.38}  & 61.2 $\pm$ 8.08 & 67.60 $\pm$ 4.52 &  
\textbf{71.66 $\pm$ 2.49}  & 50.63 $\pm$ 0.42 & 67.60 $\pm$ 4.52 & \multirow{3}{*}{100.00} \\
& 5 & \textbf{89.00 $\pm$ 1.67}& 83.4 $\pm $10.67 & 49.60$\pm$1.96 &
\textbf{96.00 $\pm$ 1.63} & 82.54 $\pm$ 0.87 & 77.60 $\pm$  2.21 \\
& 10 &  \textbf{91.60 $\pm$ 3.72} & 79.01 $\pm$ 1.34 &  50.60 $\pm$ 1.56   &
\textbf{98.00 $\pm$ 0.00} & 90.89 $\pm$ 0.22 &  84.33 $\pm$ 2.49 \\
\midrule
\multirow{3}{*}{\textbf{BA_LRP}} 
& 1 & \textbf{64.72 $\pm$ 4.44} & 49.52 $\pm$ 0.43 &  51.12 $\pm$ 2.50 &  
71.56 $\pm$ 3.62 & 54.11  $\pm$ 5.33 & \textbf{77.48 $\pm$ 1.21} & \multirow{3}{*}{97.95} \\
& 5 & \textbf{85.50 $\pm$ 2.05} & 79.01 $\pm$ 1.35  & 49.87 $\pm$ 1.28 &
\textbf{91.60 $\pm$ 1.57} & 59.21 $\pm$ 0.99  & 77.76 $\pm$ 0.52 \\
& 10 & \textbf{95.50 $\pm$ 0.50} & 56.97 $\pm$ 1.10  & 52.38 $\pm$ 1.79   &
\textbf{94.90  $\pm$ 1.09} & 66.40 $\pm$ 1.47  & 88.38 $\pm$ 1.40 \\
\midrule
\multirow{3}{*}{\textbf{Graph-Twitter}} 
& 10 & \textbf{58.13 $\pm$ 2.74}  & 49.47 $\pm$ 0.96 & 46.59 $\pm$ 5.85 &
\textbf{56.43 $\pm$ 1.39}  & 40.00 $\pm$ 3.98 & 52.40 $\pm$ 0.29 & \multirow{3}{*}{61.40} \\
& 50 & \textbf{59.73 $\pm$ 1.11} & 55.67 $\pm$ 1.04 & 50.20 $\pm$ 5.71 &
\textbf{58.93 $\pm$ 1.29} & 55.62 $\pm$ 1.12 & 52.92 $\pm$ 0.27 \\
& 100 & 53.25 $\pm$1.30 & \textbf{59.76 $\pm$ 1.00} &  56.65 $\pm$ 2.78 &
\textbf{59.51 $\pm$ 0.31} & 53.37 $\pm$ 0.55 &  55.47 $\pm$ 0.51 \\
\midrule
\multirow{3}{*}{\textbf{Graph-SST5}}
& 10 & \textbf{36.62 $\pm$ 0.76} & 28.06 $\pm$ 0.33 & 29.33 $\pm$ 3.25 &
\textbf{35.72 $\pm$ 0.65} & 25.49  $\pm$ 0.39 & 24.90 $\pm$ 0.60 & \multirow{3}{*}{44.39} \\
& 50 & 37.64 $\pm$ 0.83 & 35.96 $\pm$ 1.04  & \textbf{37.83 $\pm$ 3.62} &
\textbf{43.81 $\pm$ 0.86} & 31.47 $\pm$ 2.58  & 23.15 $\pm$ 0.35 \\
& 100 & \textbf{42.05 $\pm$ 1.35} & 41.04 $\pm$ 0.79  & 41.87 $\pm$ 1.80 &
\textbf{44.43  $\pm$ 0.45} & 32.01 $\pm$ 1.90  & 25.26 $\pm$ 0.75 \\
\bottomrule
\end{tabular}
}
\label{tab:train-time}
\end{table*}

